Text-to-speech synthesis from dark data with evaluation-in-the-loop data selection

This paper proposes a method for selecting training data for text-to-speech (TTS) synthesis from dark data. TTS models are typically trained on high-quality speech corpora that cost much time and money for data collection, which makes it very challenging to increase speaker variation. In contrast, there is a large amount of data whose availability is unknown (a.k.a, "dark data"), such as YouTube videos. To utilize data other than TTS corpora, previous studies have selected speech data from the corpora on the basis of acoustic quality. However, considering that TTS models robust to data noise have been proposed, we should select data on the basis of its importance as training data to the given TTS model, not the quality of speech itself. Our method with a loop of training and evaluation selects training data on the basis of the automatically predicted quality of synthetic speech of a given TTS model. Results of evaluations using YouTube data reveal that our method outperforms the conventional acoustic-quality-based method.

==> fig/partitioning.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp3796101352946567] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (69.92,37.88) -- (329.92,37.88) -- (329.92,49.88) -- (69.92,49.88) -- cycle ;
%Shape: Rectangle [id:dp4918154254803251] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=0.54 ] (69.92,66.88) -- (170.92,66.88) -- (170.92,76.88) -- (69.92,76.88) -- cycle ;
%Shape: Rectangle [id:dp1263454580490353] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=0.56 ] (149.92,76.88) -- (260.92,76.88) -- (260.92,86.88) -- (149.92,86.88) -- cycle ;
%Shape: Rectangle [id:dp8775963547119923] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=0.55 ] (240.92,86.88) -- (329.92,86.88) -- (329.92,96.88) -- (240.92,96.88) -- cycle ;
%Straight Lines [id:da7856899965101948] 
\draw  [dash pattern={on 6pt off 2.25pt}]  (69.92,27.88) -- (69.92,114.88) ;
%Straight Lines [id:da33561458894717244] 
\draw  [dash pattern={on 6pt off 2.25pt}]  (160.92,44.88) -- (160.92,114.88) ;
%Straight Lines [id:da5346896577295797] 
\draw  [dash pattern={on 6pt off 2.25pt}]  (250.92,43.88) -- (250.92,114.88) ;
%Straight Lines [id:da5540802931101504] 
\draw    (71.92,104.88) -- (158.92,104.88) ;
\draw [shift={(160.92,104.88)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
\draw [shift={(69.92,104.88)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da15822088877530105] 
\draw    (253.92,104.88) -- (328.92,104.88) ;
\draw [shift={(330.92,104.88)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
\draw [shift={(251.92,104.88)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da653467356994818] 
\draw    (162.92,104.88) -- (249.92,104.88) ;
\draw [shift={(251.92,104.88)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
\draw [shift={(160.92,104.88)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da21017878435256443] 
\draw  [dash pattern={on 6pt off 2.25pt}]  (329.92,27.88) -- (329.92,114.88) ;
%Straight Lines [id:da640194301012043] 
\draw    (213.92,29.88) -- (327.92,29.88) ;
\draw [shift={(329.92,29.88)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da33763840313286453] 
\draw    (177.92,28.88) -- (71.92,28.88) ;
\draw [shift={(69.92,28.88)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da24706518655532705] 
\draw    (255.92,68.88) .. controls (256.88,49.58) and (266.23,56.36) .. (283.06,59.55) ;
\draw [shift={(284.92,59.88)}, rotate = 189.46] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da10966678071540714] 
\draw    (250,69) -- (260.92,68.88) ;
\draw [shift={(260.92,68.88)}, rotate = 539.39] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;

% Text Node
\draw (104,108) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle l_{\text{cut}}$};
% Text Node
\draw (281,107) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle l_{\text{last}}$};
% Text Node
\draw (194,107) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle l_{\text{cut}}$};
% Text Node
\draw (187,20) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle l_{\text{full}}$};
% Text Node
\draw (286,53) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle l_{\text{overlap}}$};


\end{tikzpicture}


==> sec/conclusion.tex <==
\vspace{-2mm}
\section{Conclusion} \label{sec:conclusion}
\vspace{-2mm}
Under Construction

% In this paper, we propose a speech corpus construction strategy and build $1,300$ and $900$ hours data for Japanese ASR and ASV. One of our future directions is to extend the corpus to multiple languages. 

% %In this paper, we propose a speech corpus construction strategy and build $1,300$ and $900$ hours data for Japanese ASR and ASV. First, we retrieved audio and subtitles from YouTube videos with manual subtitles. Then, we constructed corpora for ASR and ASV by CTC-based cleaning and speaker variation-based cleaning. One of our future directions is to extend the corpus to multiple languages. Our method (and open-sourced scripts) is almost language-independent, so it can be easily applied to languages other than Japanese. Another direction is the use of automatic subtitles, which are 45 times larger than manual subtitles.




==> sec/corpus.tex <==
\vspace{-3mm}
\section{Corpus construction} \label{sec:data_collection}
\vspace{-2mm}

    \drawfig{t}{0.90\linewidth}{fig/overview_shortened}
    {Procedure of corpus construction.}
    All of our steps are performed with minimal language-dependent processing. \Fig{fig/overview_shortened} shows the procedure.
    
    %%% ASRU %%%
    % We describe steps to build our corpus. All the steps are performed with minimal language-dependent processing. \Fig{fig/overview_shortened} shows the procedure.

    \vspace{-2mm}
    \subsection{Data collection} \vspace{-1mm}
        % We obtain candidate data for the corpus, i.e., subtitles and audio data in the target language (Japanese in this paper) from YouTube. 
    
        \textbf{Creating search terms.} 
        The first step is to create search terms to be entered into the video search engine. We extract the target language's words with hyperlinks from HTML files of Wikipedia articles. Unlike Gigaspeech~\cite{chen2021gigaspeech}, categories are not specified, i.e., all articles are used. Also, we extract ``sudden-rise search terms'' in the past few years from Google Trends.%\footnote{\url{https://trends.google.com/}}. 
        
        \textbf{Obtaining video IDs that have subtitles.}
        Next, we retrieve video IDs that have subtitles. Entering a search word into the video search engine, we obtain a list of video ID candidates. Then, for each video, we retrieve whether the video has subtitles. In this paper, we use only manual subtitles but also make the list for automatic (i.e., machine-generated) subtitles. 
        
        \textbf{Downloading audio and caption.}
        Finally, we download the audio and manual subtitles from videos. Since the number of channels and sampling frequency of the audio file varies from video to video, we reformat the audio to 16~kHz-sampled monaural WAV format.
    
    \vspace{-2mm}
    \subsection{Specific cleansing for speech recognition} \label{sec:asr} \vspace{-1mm}
    
        The obtained audio data were already annotated with subtitles including timings.
        This dataset still included many bad samples, e.g., unspoken subtitles, English audio with Japanese subtitles, and other variations of audio--text mismatches.
        To sort-out these bad samples, we calculated a score of how well the audio segment fits to the subtitle and then filtered the utterances based on their score.
        Furthermore, as many subtitle timings were inaccurate, we fully re-aligned the subtitles to the audio.
        %
        %\paragraph{Scoring and CTC segmentation} \vspace{-1mm}
        %\label{sec:ctc_score_seg}
        To calculate a score and to re-align the subtitles to the audio, we use CTC segmentation~\cite{ctcsegmentation} as an alignment tool~\cite{ctcsegpython}. %\footnote{\url{https://github.com/lumaku/ctc-segmentation}}.
        CTC segmentation utilizes CTC log-posteriors to determine utterance timings in the audio given a ground-truth text.
        
        \textbf{Text pre--processing.}
        We apply minimal text pre--processing so that the ground truth text obtained from subtitles is composed of characters or tokens in the model dictionary.
        Numbers are replaced with their spoken equivalent using the \emph{num2words} Python library~\cite{num2words}. %\footnote{\url{https://github.com/savoirfairelinux/num2words}}.
        UTF-16 characters are mapped to the Japanese character set.
        Automated subtitles are detected and filtered out based on the average relative Levenshtein distance between subtitles.
        
        % Short description of CTC segmentation:
        \textbf{Alignment.}
        The onset and offset timings of an utterance are then estimated in three steps:
        (1) In a forward pass, transition probabilities are mapped into a trellis diagram of the ground-truth token sequence over all time steps.
        (2) Backtracking starts from the most probable timing of the last character and then determines the most probable path through the trellis.
        (3) A confidence score is derived for each utterance from the per-token probabilities in the trellis.
        The score is determined by the $L$ consecutive CTC output frames of the utterance with the lowest token probabilities; we chose $L=30$ that relates to approximately $1$s of audio.
        For a more in-depth description, readers could refer to \cite{ctcsegmentation}.
        We apply one further modification that helps with the alignment of fragmented subtitle text:
        In the original publication, the algorithm was configured to skip preambles by setting transition cost to zero for the token that marks the start of the first utterance.
        We extended this in our setup to all utterances in order to skip any unrelated audio segments.

        % explain CTC scoring here as a separate step - as it is referred to in Sec. 3.2.1
        \textbf{CTC scoring.}
        We also calculate a CTC score for each audio-text pair from its YouTube timings instead of fully aligning the subtitles to audio.
        For this, the audio segment to each subtitle is cut out to then derive its confidence score as described above.

        % confidence score length: Transformer: 768 --> 1.44s; RNN --> 0.95s
        \textbf{Cleaning.}
        Bad samples are then eliminated based on this confidence score.
        The confidence score provides an estimated log-space probability of how well the subtitles fit the audio data;
        this value is mainly influenced by the quality of ASR models, input data, and data pre-processing.
        Note that a score threshold $\theta$ of $-0.3$, used in one of our experiments, can be interpreted as a production probability of at least $75\%$ each second.
        
        \textbf{Inference of long audio files.}
        Alignment requires inference of the audio using the encoder and the CTC layer of a pre-trained ASR model.
        We found that many audio files are longer than three hours and their inference reaches a practical limitation:
        The memory complexity using a Transformer-based model is quadratic with audio length -- a device with 64 GB memory is at most able to infer $500$s of audio at once.
        Due to their rather linear memory complexity along longer audio data, RNN-based models require less memory and thus, it is possible to decode longer files.
        This can be scaled up to $2.7$h of audio until the encoding reaches a memory limit of the Pytorch toolkit.
        To overcome this limitation, we partition long audio files.
        
        %% This figure illustrates audio partitioning.
        %% Uncomment if needed (or, if you have text spacing to spare)
        %\begin{figure}[t]
        %\centering
        %\input{fig/partitioning}
        %\vspace{-2mm}
        %\caption{Partitioning of longer audio files to smaller parts.}
        %\vspace{-4mm}
        %\label{fig:partitioning}
        %\end{figure}
        
        %% More detailed description of partitioning, uncomment if needed.
        %Partitioning is done by splitting the audio into smaller blocks, performing inference on the parts, and then concatenating the posteriors to perform CTC segmentation.
        %A long audio file of length $l_{\text{full}}$ samples is partitioned into parts with length $l_{\text{cut}}$.
        %The maximum length of the last part is chosen to $l_{\text{last}}\leq  1.25\cdot l_{\text{cut}}$ to prevent too short audio parts at the end.
        %For our experiments, $l_{\text{last}}$ includes up to $320$s of audio.
        %As abrupt cuts in the audio cause distortions during inference, we add an overlap of length $l_{\text{overlap}}$ to each side of the block.
        %By inspection of CTC posteriors, an overlap of at least $600$ms is required to reduce distortions and impact on scoring to an acceptable level.
        %we chose a value corresponding to $1$s of audio. % comment: this value results in different durations depending on model, see comment about confidence score length above
        %Before concatenating the inferred posteriors of the parts, the CTC layer outputs that relate to the overlaps are omitted.
        %All lengths were chosen as multiples of the samples--to--posteriors ratio to preserve timing information and ensure the correct shape of the concatenated CTC posterior tensor.

        Partitioning is done by splitting the audio into smaller blocks, performing inference on the parts, and then concatenating CTC posteriors.
        Maximum block sizes were chosen depending on the memory consumption of the model and available memory;
        the last block may be $25\%$ longer to avoid too short blocks.
        As abrupt cuts in the audio cause distortions during inference, we add an overlap to each side of the block; overlapping posteriors are later omitted for scoring.
        By inspection of CTC posteriors, an overlap of at least $600$ms is required to reduce impact of partitioning on scoring to an acceptable level.
        All lengths were chosen as multiples of the samples--to--posteriors ratio to preserve timing information and ensure the correct shape of the concatenated CTC posterior tensor.

    
    \subsection{Specific cleansing for speaker verification} \label{sec:asv} \vspace{-1mm}
        Unlike an ASR corpus, ASV requires high-quality speaker labels. Therefore, we propose an unsupervised method for only extracting monologue videos (i.e., single-speaker videos) from the obtained videos. Furthermore, we remove videos with text-to-speech (TTS) voices, which have different characteristics from natural speech.
            
        \drawfig{t}{0.60\linewidth}{fig/single-speaker-collection}
        {Comparison of distributions in speaker space.}

        %\vspace{-1mm}
        %\subsubsection{Removing non-speech and too-short videos}  \vspace{-1mm}
        \textbf{Removing non-speech and too-short videos.}
        First, we delete videos without speech. Unlike the corpus for ASR, there is no need to align subtitle and speech. Therefore, we simply use voice activity detection (VAD) here. We applied VAD to sections trimmed out based on the subtitles and used only sections mainly consisting of speech. Also, too-short videos are deleted. This is for robustly calculating the intra-video statistics described below.
        
        %\vspace{-1mm}
        %\subsubsection{Evaluating intra-video variation in speaker space}  \vspace{-1mm}
        \textbf{Evaluating intra-video variation in speaker space.}
        To extract single-speaker videos, we compute the speaker variability in the video. \Fig{fig/single-speaker-collection} illustrates the concept. We use the $d$-vector~\cite{variani14dvecs}, deep learning-based speaker representation, which is extracted using pre-trained models. The $d$-vector is first calculated for each utterance. Then, the variance of the $d$-vectors is calculated within the video. We expect that the variance of TTS voices becomes smaller than the single-speaker voices because the TTS voice has no fluctuation among utterances. Also, if the different speakers' voices are contaminated (i.e., multi-speaker video), the variance will become larger than the single-speaker video. Therefore, we can eliminate TTS videos and multi-speaker videos by setting the appropriate threshold to the variance. For implementation, the $d$-vector is reduced to a lower dimension by t-SNE~\cite{maaten08tsne}, and the determinant of its covariance matrix is obtained.
            
            %%% ASRU %%%
            %To extract single-speaker videos, we compute the speaker variability in the video. \Fig{fig/single-speaker-collection} illustrates the concept of evaluating intra-video variation in speaker space. We use the $d$-vector~\cite{variani14dvecs}, deep learning-based speaker representation, which is extracted using pre-trained models. The $d$-vector is first calculated for each utterance trimmed out based on the subtitles. Then, the variance of the $d$-vectors is calculated within the video. We expect that the variance of TTS voices becomes smaller than the single-speaker voices because the TTS voice has no fluctuation between utterances. Also, if the different speakers' voices are contaminated (i.e., multi-speaker video), the variance will become larger than the single-speaker video. Therefore, we can eliminate TTS videos and multi-speaker videos by setting the appropriate threshold to the variance. For implementation, the $d$-vector is reduced to a lower dimension by t-SNE~\cite{maaten08tsne}, and the determinant of its covariance matrix is obtained.
        
        %\vspace{-1mm}
        %\subsubsection{Grouping videos by YouTube Channel ID} \vspace{-1mm}
        \textbf{Grouping videos by YouTube Channel ID.}
        It is necessary to prevent the same speaker from being counted as different speakers. We obtain and use the YouTube Channel ID of each video. Single-speaker videos with the same Channel ID are grouped together and considered as a unique speaker. 
    

==> sec/experiment.tex <==
\vspace{-2mm}
\section{Experimental evaluation} \label{sec:experiment}
\vspace{-2mm}
Under Construction
% 実験条件（コーパス、学習に使ったパラメータなど）
%   母語推定機（Classifier lossの話はここ）（短く）
% 評価
%   男女軸、「L2っぽさ」、「自然性」
%   日本人対象の日本語音声合成に対する評価
%   図は必要

% 客観評価
%   Speaker Generationで学習した分布の評価（元論文みたいに話者生成できているか）s-g, g-g, s-s
%   補間分布のg-g
%   属性間g-g（別の分布で一番近い話者）（遷移しているのを客観評価で見せたい）
%   （スペースがあったら）classifierを使った属性評価

%     \subsection{Evaluation in data collection} \vspace{-1mm}
%         The period of data collection was between February and April of 2021. From the data collection results listed in \Table{corpus_spec}, we can describe 1) $5.09$ videos are found for each search term and 2) $0.92$~\% of videos have manual subtitles, and $41.7$~\% have automatic subtitles. In the end, we obtained approximately $10,000$ hours of speech data from $110,000$ YouTube videos. % Most of the videos are less than 5 minutes long, and the average duration is 3.8 minutes. Also, almost all utterances are shorter than 25 seconds because the subtitles are synchronized with the video. 
        
%         %%% ASRU %%%
%         % The video data was collected between February and April of 2021. Also, the Wikipedia timestamp used to create search terms was February 2021. \Table{corpus_spec} lists the number of search terms and videos we collected. From these numbers, we can describe that
%         % \begin{itemize} \leftskip -5mm \itemsep -1mm
%         %     \item $5.09$ videos are found for each search term.
%         %     \item $0.92$~\% of videos have manual subtitles, and $41.7$~\% have automatic subtitles.
%         % \end{itemize}
%         % In the end, we obtained approximately 10,000 hours of speech data from 110,000 YouTube videos. \Fig{fig/duration} shows duration of videos and utterances. Most of the videos are less than 5 minutes long, and the average duration is 3.8 minutes. Also, a few videos are several hours long but these are very rare. On the other hand, almost all utterances are shorter than 25 seconds because the subtitles are synchronized with the video, but a few utterances are several hours long. 
 
%         \input{tab/corpus_spec}
%         \input{tab/corpus_comparison}

%         %\drawfig{t}{0.9\linewidth}{fig/duration}
%         %{Duration of found videos and its statistics.}

%         \Table{corpus_comparison} shows a comparison with the existing corpus. The duration of our corpus is a subset used in the ASR or ASV experiments described below. Among ASR corpora, our corpus is similar in size to LaboroTVspeech (Ja)~\cite{ando21laborotvspeech} and Common Voice (En)~\cite{ardila20commonvoice}. Also, among ASV corpora, it is the first open-source Japanese corpus and is similar in size to CN-Celeb (Zh)~\cite{fan19cnceleb}. 
        
%         %%% ASRU %%%
%         % \Table{corpus_comparison} shows a comparison with the existing corpus. The duration of our corpus is not all of the collected data described above but subsets used in the ASR and ASV experiments described below. Among ASR corpora, our corpus is similar in size to LaboroTVspeech (Japanese)~\cite{ando21laborotvspeech} and Common Voice (English)~\cite{ardila20commonvoice}. Also, among ASV corpora, it is the first open-source Japanese corpus and is similar in size to CN-Celeb (Chinese)~\cite{fan19cnceleb}. We are planning to further analyze the collected data and expand the corpus size.


%     \subsection{Evaluation in speech recognition} \vspace{-1mm}
%         %\subsubsection{Data cleaning} \vspace{-1mm}
%         %\label{sec:data_cleaning}
%         \textbf{Data cleaning.}
%         The most important data pre-processing is to prune utterances that have the wrong transcriptions and fix the incorrect timing.
%         We consistently employed CTC segmentation and CTC scoring, as described in Section \ref{sec:asr}.
%         We used a pre-trained CTC model based on the ESPnet LaboroTVspeech~\cite{ando21laborotvspeech} recipe~\cite{Laborotvrecipe}. %\footnote{\url{https://github.com/espnet/espnet/tree/master/egs2/laborotv/asr1}}. 
%         Table \ref{tab:asr_data_stats} summarizes the statistic of the various training and test sets.
        
        
%         %As a pilot study, we used two subsets of our corpus:
%         %\begin{itemize}
%         %    \item "single\_speaker" (or "ss" in short): based on the single speaker subset, as described in Section \ref{sec:asv}
%         %    \item "top\_15k" (or "15k" in short): extracted based on top 15,000 videos in terms of the average score for each video.
%         %\end{itemize}
%         As a pilot study, we used two subsets of our corpus:
%         (1) "single\_speaker" (or "ss" in short) based on the single speaker subset, as described in Section \ref{sec:asv}, and
%         (2) "top\_15k" (or "15k" in short) extracted based on top 15,000 videos in terms of the average score for each video.
%         %The total file size of the single\_speaker and top\_15k subsets including the silence region amounts to 100GB and 300GB, respectively.
%         Note that top\_15k is pruned only based on utterance confidence scores and it may contain multi speaker videos, unlike single\_speaker.
%         Also a part of these subsets is overlapped.
        
%         \drawfig{t}{0.85\linewidth}{fig/hist_score_L20}
%         {Histograms of the score for different ASR models over all utterances of top\_15k.} %, with a scoring length that corresponds to $0.96$s of audio.}

%         These subsets are further decomposed into the training and test sets, which will be explained in the next section.
%         We also prepare the various training sets by changing the threshold value $\theta$ of the confidence score obtained by CTC segmentation for the single\_speaker and top\_15k subsets.
%         To determine the threshold value, we investigate the distribution of the confidence score over all utterances in the top\_15k subset, as shown in \Fig{fig/hist_score_L20}.
%         This distribution clearly shows that the peak of the distribution starts around -3.0 in both RNN and transformer based CTC models.
%         Based on the observation, we regard the utterances located in the wide-based region as outlier data points, and use -3.0 as the lowest threshold for pruning in Table~\ref{tab:asr_data_stats}.
%         The largest training set is obtained by combining the single\_speaker and top\_15k subsets (train\_ss\_15k).
%         % It contains more than 17 thousand videos, 1.2 million utterances, and 1.3 thousand hours\footnote{We can further scale up our training data up to approximately five times more if we use the entire corpus.}.
        
%         %\subsubsection{Test set design} \vspace{-1mm}
%         %\label{sec:test_set_design}
%         \textbf{Test set design.}
%         %We carefully designed a test set for ASR evaluation from our corpus.
%         Focusing on the "single\_speaker" videos reduces the cost of manual process of verifying audio and transcriptions.
%         The rest of the procedure is as follows:
%             (1) Select 1,621 videos from the "single\_speaker" videos that include "easy" utterances scored more than -0.3 threshold value based on CTC.
%             (2) Randomly pick up 324 videos, around 20\%, and use them as a test video set, which has 3,396 easy utterances in total.
%             (3) Manually listen utterances and identify 1,614 utterances having correct transcriptions.
%             (4) Split them into the development \textbf{dev\_easy\_jun21} and evaluation \textbf{eval\_easy\_jun21} sets, which have 785 and 829 utterances, respectively.
%         %First, we only focused on the "single\_speaker" videos to reduce the cost of manual process of verifying the audio and corresponding correct transcriptions.
%         %The rest of the procedure is as follows:
%         %\begin{enumerate}
%         %    \item Select 1,621 videos from the "single\_speaker" videos that include "easy" utterances scored more than -0.3 threshold value based on CTC.
%         %    \item Randomly pick up 324 videos (around 20\%) and use them as a test video set, which has 3,396 easy utterances in total.
%         %    \item Manually listen utterances and identify 1,614 utterances having correct transcriptions.
%         %    \item Split them into the development (\textbf{dev\_easy\_jun21}) and evaluation (\textbf{eval\_easy\_jun21}) sets, which have 785 and 829 utterances, respectively.
%         %\end{enumerate}
%         We also made an additional test set with "normal" utterances\footnote{
%         The definition of "easy" and "normal" test sets are determined based on the CTC score objectively. Our listening process and later ASR experiments confirmed that this categorization is reasonable.
%         } scored more than $-1.0$ threshold value.
%         We fixed to use the same test video set as we defined before, and performed steps 3 and 4.
%         We made \textbf{dev\_normal\_jun21} and \textbf{eval\_normal\_jun21} sets, which have 1,036 and 834 utterances, respectively.
%         %We will perform the above procedure for the different threshold value or non single\_speaker subsets to create more difficult (e.g., hard) test sets in the future.

%         \begin{table}[t]
%             \centering
%             \footnotesize
%             \caption{Training and test data statistics for the ASR task. $\theta$ is a threshold used to prune bad utterances based on the CTC score.}
%             \label{tab:asr_data_stats}
%             \begin{tabular}{c|rrrr}
%             & $\theta$ & \# videos & \# utts & hours \\
%             \hline
%             dev\_easy\_jun21       & -0.3 & 110   & 785     & 0.7 \\
%             eval\_easy\_jun21      & -0.3 & 106   & 829     & 0.7 \\
%             dev\_normal\_jun21     & -1.0 & 128   & 1,036   & 1.1 \\
%             eval\_normal\_jun21    & -1.0 & 129   & 834     & 0.8 \\
%             \hline
%             train\_single\_speaker & -0.3 & 1,297 & 14,797  & 12.7 \\
%             train\_single\_speaker & -0.5 & 1,792 & 26,209  & 24.2 \\
%             train\_single\_speaker & -1.0 & 2,906 & 66,563  & 71.9 \\
% %            train\_single\_speaker & -2.0 & 4,068 & 186,733 & 227.4 \\
%             train\_single\_speaker & -3.0 & 4,342 & 285,846 & 362.0 \\
%             \hline
%             train\_top\_15k & -3.0 & 14,418 & 1,048,699 & 1087.1 \\
%             \hline
%             train\_ss\_15k & -3.0 & \textbf{17,761} & \textbf{1,270,124} & \textbf{1376.9} \\
%             \end{tabular}
%             \vspace{-4mm}
%         \end{table}

%         %\subsubsection{ASR models} \vspace{-1mm}
%         \textbf{Experimental results.}
%         We used an ESPnet state-of-the-art conformer model \cite{gulati20conformer,guo2021recent} based on hybrid CTC/attention architectures \cite{watanabe20202020}.
%         %The conformer encoder has 12 conformer blocks with a kernel size of 31 and the transformer decoder has 8 blocks.
%         %Encoder and decoder blocks each have 512 attention dimensions, 8 attention heads, and $2,048$ feed forward dimensions.
%         %We used SpecAugment during training \cite{park2019specaugment}.
%         %Inference was performed without LM.
%         %We did not use LM shallow fusion during inference.
%         The detailed configuration can be found in the ESPnet JTubeSpeech recipe. %\footnote{\url{https://github.com/espnet/espnet/pull/3311}}. % OR: ~\cite{jtubespeechpullrequest}

%         %\subsubsection{Experimental results} \vspace{-1mm}
%         %\textbf{Experimental results.}
%         \Fig{fig/cer_hour2} shows the ASR performance for various amounts of training data by changing the score threshold $\theta$.
%         We confirmed that the normal test set was more difficult than the easy test set.
%         %(the error rate was increased by 1.6 to 2.1 times more).
%         This result validates our design of the test set by controlling the difficulties based on the score.
%         As regards the amounts of training data, if we increase the amount of training data by reducing $\theta$, the training data may contain more noisy transcriptions or distorted audio segments.
%         Nevertheless, the ASR performance was improved, and the final CERs were $5.2\%$ in eval\_easy\_jun21 and $10.7\%$ in eval\_normal\_jun21.
%         These CER ranges are similar to other Japanese ASR benchmarks, e.g., $4-6\%$ in CSJ \cite{maekawa00csj} and $13\%$ in LaboroTVspeech \cite{ando21laborotvspeech}.
%         %Thus, we can conclude that our ASR benchmark is reasonable as our initial step of the corpus design.
%         We also list the largest training data case (ss\_15k\_1376h) by combining the single\_speaker subset and top\_15k subsets.
%         %This data was obtained by combining the single\_speaker subset and the top\_15k subset, which contains multi-speaker recordings. %, as described in Section \ref{sec:data_cleaning}. 
%         The performance was improved in most cases except for dev\_easy\_jun21.
%         %possibly due to the mismatch between single speaker and multi-speaker recordings.
%         %The eval\_normal\_jun21 CER was improved from $10.7\%$ to $10.0\%$.
%         This result confirms that 
%         %while we need more careful cleaning to maintain the clean speech recognition task performance, 
%         more training data is generally helpful to improve the performance of more challenging data.
        
%         \drawfig{t}{0.98\linewidth}{fig/cer_hour2}
%         {ASR performance for various amounts of training data (12, 24, 71, 362, and 1376 hours) by changing the score threshold and combining multi-speaker recordings. 
%         %See Table \ref{tab:asr_data_stats} for the detailed training data information.
%         } 
    
%         Finally, we evaluate the effectiveness of CTC segmentation, as discussed in Section \ref{sec:asr}.
%         We used train\_single\_speaker with $-1.0$ score threshold (71.9 hours) and prepared the corresponding training data based on the original YouTube timings only with CTC scoring.
%         Table \ref{tab:ctc_seg} shows that the CTC segmentation significantly improved the performance and shows the effectiveness of the re-aligning for the YouTube audio data, as suggested by \cite{chen2021gigaspeech}.
    
%         \begin{table}[t]
%             \centering
%             \footnotesize
%             \caption{The effectiveness of CTC segmentation.}
%             \label{tab:ctc_seg}
%         \begin{tabular}{l|cr|cr}
%                                          & dev\_easy                     & \multicolumn{1}{c|}{dev\_normal} & dev\_easy                    & \multicolumn{1}{c}{dev\_normal} \\ \hline
%         \multicolumn{1}{r|}{original timing} & \multicolumn{1}{r}{11.5} & 16.5                        & \multicolumn{1}{r}{9.2} & 15.7                       \\
%         \multicolumn{1}{r|}{CTC segmentation}  & \multicolumn{1}{r}{\textbf{9,2}}  & \textbf{14.3}                       & \multicolumn{1}{r}{\textbf{6.9}} & \textbf{13.6}                      
%         \end{tabular}
%         \vspace{-4mm}
%         \end{table}    
    
%     \vspace{-1mm}
%     \subsection{Evaluation in speaker verification} \vspace{-1mm}
%         \subsubsection{Data cleansing} \vspace{-1mm}
%         We used py-webrtcvad\footnote{\url{https://github.com/wiseman/py-webrtcvad}} for VAD and a pre-trained model\footnote{\url{https://github.com/yistLin/dvector}} for extracting $d$-vectors. The variation in speaker space was computed from more than 10 utterances for each video. As a pilot study, we used randomly selected 35,000 videos (approx. 30\% of total). \Fig{fig/tsne_score_rev} shows two levels of rapid increase: near 0 and near 8 to 9 on the x-axis. Following the concept in \Fig{fig/single-speaker-collection}, we set a threshold around these levels and assign ``TTS,'' ``single speaker,'' or ``multi speakers,'' class to the videos.
        
%         %%% ASRU %%%
%         % We used py-webrtcvad\footnote{\url{https://github.com/wiseman/py-webrtcvad}} for VAD and an open-sourced pre-trained model\footnote{\url{https://github.com/yistLin/dvector}} for extracting $d$-vectors. The intra-video variation in speaker space was computed from more than 10 utterances for each video. As a pilot study, we used randomly selected 35,000 videos (approx. 30\% of total).

%         %%% ASRU %%%
%         % \Fig{fig/tsne_score_rev} shows the log determinant of a covariance matrix of $d$-vectors in each video (i.e., intra-video variation). In this figure, we can see two levels of rapid increase. The first level is near 0 on the x-axis, which means that videos with extremely low variance are included in the collected data. The second level is near 8 to 9 on the x-axis. Following the concept in \Fig{fig/single-speaker-collection}, we set a threshold around these levels and assign ``TTS,'' ``single speaker,'' or ``multi speakers,'' class to the videos, starting from the lowest value.
    
%         \drawfig{t}{0.7\linewidth}{fig/tsne_score_rev}
%         {The intra-video variation in speaker space}    

%         We quantitatively evaluate the authenticity of this classification. We randomly extracted 100 videos from each class and annotated a true class label. 
%         %Multi-TTS videos (i.e., multiple TTS systems) and overdubbed-voice videos (e.g., overdubbed singing voices) were annotated as ``multi speakers.'' 
%         Multi-TTS videos and overdubbed-voice videos were annotated as ``multi speakers.'' 
%         To accurately find TTS videos, a TTS specialist participated in this annotation. \Table{video_type} shows that each class has their suitable videos. Especially, the ``single speaker'' class does not contain multi-speaker videos. Therefore, our method works for choosing the single-speaker videos. Some single-speaker videos leak to the ``TTS'' class, but this impact is limited because the ``TTS'' class has only a few videos.
        
%         %%% ASRU %%% 
%         % \Table{video_type} lists the result. It is observed that each class has their suitable videos. Especially, the ``single speaker'' class does not have multi-speaker videos. Therefore, we can demonstrate that our method works for eliminating the multi-speaker videos and choosing the single-speaker videos. Some single-speaker videos leak to the ``TTS'' class, but this impact is limited because the ``TTS'' class has only a few videos.

%         \input{tab/video_type}

%         \subsubsection{ASV dataset design and models} \vspace{-1mm}
%         %For considering the usage of the same evaluation sets as ASR, we designed the evaluation trials from the ASR evaluation set (\textbf{eval\_easy\_jun21)}.  
%         From the single-speaker videos, 92 unique speakers were selected as the enrollment and testing speakers. For the training and development datasets, 1,795 unique speakers were selected.
%         %Then, we selected 1,795 unique speakers for a training dataset and development one %from the single-speaker videos except for the videos of the 92 speakers. Consequently, 3498 videos were used for training and development datasets. 
%         In the training, 127,997 and 25,392 utterances were used for training and development datasets, respectively. 
%         In the testing, we designed an enrollment utterance and a testing one were picked up from the same video but different segments. %For picking up the test utterances accurately, the manual subtitle information was used. 
%         In the testing, we performed 25,392 trial pairs, included 276 correct pairs and 25,116 incorrect pairs.

%         %\subsubsection{ASV models} \vspace{-1mm}      
%         We used a speaker embedding network, which was built with four convolutional neural networks, pooling layers and two full connected layers. %The output of the final layer was regarded as a speaker embedding vector. 
%         As the input feature, 40-order Mel-Frequency Cepstrum Coefficients with 25-ms frame length and half overlapped shift were used. The speaker-embedding vector was 512 dimensions. The evaluation metric is equal error rate (EER) was used for our evaluation by comparing the cosine distance.
%         %The speaker embedded vectors extracted from the enrollment utterances and the testing utterance were compared by the cosine distance similarity. Equal error rate (EER) was used for our evaluation.

%         \subsubsection{ASV performance} \vspace{-1mm}
%         We performed ASV evaluations, and the EER of our ASV system with JTubeSpeech was \textbf{10.9\%}.  Our system was regarded as the speaker embedding system based on the CNN-based model. Even though such a simple system, this result had the similar performance to the CNN-based model (VGG-M) trained with Voxceleb1~\cite{nagrani19voxceleb}.
%         As a pilot study, we designed a simple benchmark. For example, the result was obtained with the small model and probabilistic linear discriminant analysis (PLDA) scoring and data augmentation techniques were not performed. %Since the trial pairs of the correct cases were picked up from the same video in the correct pair cases, some trial part seemed to be easy. 
%         However, from this simple benchmark, we could show the techniques of data cleaning for selecting a unique speakers and 
%         constructing ASV systems performed well. Consequently, we established the Japanese ASV systems with large-scale open source media in the first time.
% %        because of the dataset came from Youtube videos, there were hevy BGM and sound effects. The 
        

% %        Table \ref{tab:asv_results} shows the EER of our ASV system with JTubeSpeech. As a pilot study, we designed a simple benchmark. For example, the result was obtained with a small model and probabilistic linear discriminant analysis (PLDA) scoring and data augmentation techniques were not performed. Since the trial pairs were picked up from the same video in the correct pair cases, some part seemed to be easy.         

% %        To fully utilize YouTube videos for estimating reliable ASV systems, data augmentation and speech enhancement techniques and other data cleaning schemes will be required. In addition, as shown in Table \ref{tab:video_type}, some TTS speakers remained in the single speakers dataset. We will discuss the influences of including TTS speakers and how to eliminate such speakers. To keep the reproducibility of our ASV system, we will add the ASV recipe based on the ESPnet style in the future.

% \begin{comment}
%     \begin{table}[t]
%         \centering
%         \caption{EER (\%) of ASV evaluation.}
%         \label{tab:asv_results}
%         \begin{tabular}{c|r}
%         & eval\_easy\_jun21  \\
%         \hline
%         Spk embeddings / cosine dist. & 10.9\% 
%         \end{tabular}
%     \end{table}  
% \end{comment}
        
    

==> sec/introduction.tex <==
\vspace{-2mm}
\section{Introduction} \label{sec:introduction}
\vspace{-2mm}
Under Construction
% 音質が向上して多話者の追求もなされる中で、話者生成とは（概要と意義）
% 先行手法としてのTacoSpawnの紹介。この手法は発展の余地を残して発表されたものである。そして、話者生成のために話者を分布として保持する考え方は確率分布に対する既存の手法を適用できる可能性を持っていた。話者の分布を混ぜることで、Mid-attributeな属性を持つ話者の音声を合成する。（ここでMid-attributeの説明）応用としては例えば、L2教育など。
% そこで、この論文では分布の混合をする。（Optimal transport for Gaussian mixture models）混合を試すにあたり、話者の性別とコーパスの言語（話者の母語として捉える）を使用した。（アブストに1、2行足したくらいの情報量）
% 主観評価をして、その結果として混合した分布から元の分布に属する話者の属性を混合したような話者が得られることがわかった（予定）例えば、L1らしい→L2らしい（Non-nativeness）と遷移する話者分布。
% この論文の貢献は「話者分布混合による中間的な属性の話者の獲得」「知覚的にも中間的な属性を持つことの実験による確認」


% Japanese, the target language in this paper, is also this example. The CSJ corpus~\cite{maekawa00csj} is the most frequently used corpus for Japanese ASR, but its size is relatively small ($600$~ hours) compared to modern English corpora such as Common Voice~\cite{ardila20commonvoice} ($1,100$~hours). Also, the modern size of ASV corpora is more than $1,000$ hours~\cite{nagrani19voxceleb,fan19cnceleb}, but there is no open-sourced corpus for Japanese ASV.

% To construct a large-scale corpus, several studies have collected text-audio pairs from videos~\cite{abuelhaija16youtube8m,nagrani19voxceleb,oneill21spgispeech,galvez2021peoplespeech}.
% For example, YouTube provides videos in diverse genres, recording environments, speakers, and language accents. There is no doubt that such \textit{in-the-wild} data is useful for wide purpose of modern speech technology. Chen~\cite{chen2021gigaspeech} proposed a strategy to collect English videos for ASR use. Also, Fan~\cite{fan19cnceleb} manually selected Chinese celebrities and extracted videos for ASV use. Unlike these methods that require language-dependent and manual processes, this paper aims to develop a corpus with almost no language-dependent and no manual processes. The establishment of this method will be useful for building corpora of many languages, not limited to English and Chinese.

% %%% ASRU %%%
% % To construct a large-scale speech corpus, several studies have collected text-audio pairs from videos~\cite{abuelhaija16youtube8m,nagrani19voxceleb,oneill21spgispeech,galvez2021peoplespeech}. For example, YouTube provides videos in diverse genres, recording environments, speakers, and language accents. There is no doubt that such \textit{in-the-wild} data is useful for wide purpose of modern speech technology, e.g., ASR and ASV. Chen~\cite{chen2021gigaspeech} proposed a strategy to collect category-specific English videos for ASR use. They manually defined 24 categories and selected videos with manual (i.e., human-generated) captions. Also, Fan~\cite{fan19cnceleb} manually selected 1,000 Chinese celebrities and extracted videos of those people. Unlike these methods that require language-dependent and manual processes, this paper aims to develop a corpus with almost no language-dependent and no manual processes. The establishment of this method will be useful for building corpora of many languages, not limited to English and Chinese.

% In this paper, we propose a mostly language-independent strategy to construct a speech corpus for both ASR and ASV, and then construct a Japanese speech corpus ``JTubeSpeech'' by using the proposed method. We first crawl YouTube in order to generate candidate audio-text pair data. For ASR, the subtitles are aligned to the audio using a CTC-based ASR model using CTC segmentation~\cite{ctcsegmentation}. This method calculates a confidence score to filter the audio-text pair~\cite{ctcsegmentation,zhang2021nemo,bakhturina2021hifi}. Unlike the conventional hidden Markov model (HMM) based cleaning \cite{trmal2017kaldi,guo2021recent}, this method does not require any language-dependent pre-processing thanks to the end-to-end framework. 
% Also, for ASV, the audio can be filtered by calculating variation of speaker representation within a video. This paper applies the above techniques to a Japanese corpus as a case study. Experimental evaluation demonstrates 1) we designed a new Japanese ASR benchmark with more than 1,300 hours of training data and the official test sets, and 2) we also constructed 900 hours of Japanese ASV corpus. The contributions of this work are as follows:
%     \vspace{-2mm}
%     \begin{itemize} \leftskip -5mm \itemsep -1mm
%         \item We construct a new modern-size corpus for Japanese ASR and ASV from YouTube videos. The video list is open-sourced in our project page\footnote{\url{https://github.com/sarulab-speech/jtubespeech}}.
%         \item Our process is applicable to many languages with high reproducibility. The repository also contains the script, which has been extended to support multiple languages for the data collection.
%     \end{itemize}
%     \vspace{-2mm}

% %%% ASRU %%%
% % In this paper, we propose a mostly language-independent strategy to construct a speech corpus for both ASR and ASV, and then construct a Japanese speech corpus ``JTubeSpeech'' by using the proposed method. We first create a large number of search terms and crawl YouTube in order to generate candidate data for the corpus. For ASR, the subtitles are aligned to the audio using a CTC-based ASR model using CTC segmentation~\cite{ctcsegmentation}.
% % This method also calculates a confidence score for each subtitle that quantifies how well it fits to the corresponding audio segment.
% % Audio-text pairs can then be filtered based on a chosen confidence score threshold~\cite{ctcsegmentation,zhang2021nemo,bakhturina2021hifi}.
% % Compared with the conventional hidden Markov model (HMM) based cleaning \cite{trmal2017kaldi,guo2021recent}, this method does not require the pronunciation dictionary and other language-dependent pre-processing thanks to the end-to-end framework.
% % Also, the data is cleansed based on speaker variation for ASV use. The audio can be filtered by calculating variation of speaker representation within a video.
% % This paper applies the above techniques to a Japanese corpus as a case study, but almost all process steps are language independent. Experimental evaluation demonstrates 1) 10,000 hours data were collected from videos with manual subtitles, 2) we consistently employed CTC-based techniques for data cleaning with minimal language-dependent processing and designed a new Japanese ASR benchmark with more than 1,300 hours of training data in total and the official test sets, 3) we proposed a speaker variation-based technique for data cleansing without language dependency and constructed 900 hours of corpus for Japanese ASV. The contributions of this work are as follows:
% %     \begin{itemize} \leftskip -5mm
% %         \item We construct a new modern-size corpus for Japanese ASR and ASV from YouTube videos. A video list we collected is open-sourced in \url{https://github.com/sarulab-speech/jtubespeech}.
% %         \item Our process is applicable to many languages with high reproducibility, not limited to Japanese because it has only minimal language-dependent processing. The above repository also contains the script, which has been extended to support multiple languages for the data collection part.
% %     \end{itemize}

==> sec/model.tex <==
\vspace{-3mm}
\section{Proposed Method} \label{sec:model_construction}
\vspace{-2mm}
Under Construction
% model construction
%   Multi-SpeakerかつMulti-lingualなFastSpeech2とSpeaker Generationモジュール、Loss関数
% Speaker Distributions Mixing
%   式を書く（コスト計算式、ガウシアンの中間、重み計算のための最小化対象）
%   変数の書き直しがいるのと、属性に対応するGMMがあることを明示。最初に変数を明示。
% 話者生成
%   Mixingで得た分布からベクトルをサンプリング。Look-up tableの話者エンベディングの代わりに使用。


==> sec/related-work.tex <==
\vspace{-3mm}
\section{Related works} \label{sec:relatd-work}
\vspace{-2mm}
Under Construction
% Multi-Speaker FastSpeech2
% TacoSpawn
% Optimal transport for Gaussian mixture models
%   Optimal transport自体の説明から入る

==> tab/corpus_comparison.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \caption{Comparison of speech corpora of Japanese (upper half) and other rich-resource languages (lower half).}
    \begin{tabular}{c|cccc}
    Lang.            & Task          & Corpus                             & Open-source & Duration \\ \hline
    Ja            & ASR/ASV       & JNAS~\cite{itou99jnas}                & No        & 90       \\
    Ja            & ASR           & CSJ~\cite{maekawa00csj}               & No        & 600 \\
    Ja            & ASR           & LaboroTVspeech~\cite{ando21laborotvspeech}  & Yes       & 2,000 \\
    Ja            & ASR           & Common Voice~\cite{ardila20commonvoice} & Yes  & 2 \\ 
    Ja            & ASV           & Liveness~\cite{shiota15liveness}      & No        & 4 \\
    Ja            & ASR/ASV       & \textbf{JTubeSpeech (ours)}           & Yes       & 1,300/900 \\ \hline
    En             & ASR           & Librispeech~\cite{panayotov2015librispeech} & Yes  & 982 \\    
    En             & ASR           & Common Voice~\cite{ardila20commonvoice} & Yes  & 1,100 \\
    En             & ASR           & SPGISpeech~\cite{oneill21spgispeech} &  Yes       & 5,000 \\ 
    En             & ASR           & GigaSpeech~\cite{chen2021gigaspeech}  & Yes       & 10,000 \\
    En    & ASV           & VoxCeleb~\cite{nagrani19voxceleb}     & Yes       & 2,800 \\ 
    Zh             & ASR           & Common Voice~\cite{ardila20commonvoice} & Yes & 12 \\
%    Zh             & ASR           & HKUST~\cite{liu06hkust}               & No        & 200 \\
    Zh             & ASR           & AISHELL-2~\cite{du18aishell2}         & Yes       & 1,000 \\
    Zh             & ASV           & CN-Celeb~\cite{fan19cnceleb}          & Yes       & 1,000 \\
    \end{tabular}
    \label{tab:corpus_comparison}
    \vspace{-4mm}
\end{table}


% \begin{table*}[t]
%     \centering
%     \footnotesize
%     \caption{Comparison of speech corpora of Japanese (upper half) and other rich-resource languages (lower half).}
%     \begin{tabular}{c|ccccc}
%     Language            & Task          & Corpus                                & Source                & Open-source & Duration [hour] \\ \hline
%     Japanese            & ASR/ASV       & JNAS~\cite{itou99jnas}                & In-house recording    & No        & 90       \\
%     Japanese            & ASR           & CSJ~\cite{maekawa00csj}               & Conference talk       & No        & 600 \\
%     Japanese            & ASR           & LaboroTVspeech~\cite{ando21laborotvspeech} & Broadcast TV     & Yes       & 2,000 \\
%     Japanese            & ASR           & Common Voice (ja)~\cite{ardila20commonvoice} & Web-based recording & Yes  & 2 \\ 
%     Japanese            & ASV           & Liveness~\cite{shiota15liveness}      & In-house recording    & No        & 4 \\
%     Japanese            & ASR/ASV       & \textbf{JTubeSpeech (ours)}           & YouTube               & Yes       & 1,300/900 \\ \hline
%     English             & ASR           & Librispeech~\cite{panayotov2015librispeech} & Web-based recording & Yes  & 982 \\    
%     English             & ASR           & Common Voice (en)~\cite{ardila20commonvoice} & Web-based recording & Yes  & 1,100 \\
%     English             & ASR           & SPGISpeech~\cite{oneill21spgispeech}  & Earnings call       & Yes       & 5,000 \\ 
%     English             & ASR           & GigaSpeech~\cite{chen2021gigaspeech}  & Web crawl             & Yes       & 10,000 \\
%     English (mostly)    & ASV           & VoxCeleb~\cite{nagrani19voxceleb}     & YouTube               & Yes       & 2,800 \\ 
%     Chinese             & ASR           & Common Voice (cn)~\cite{ardila20commonvoice} & Web-based recording & Yes & 12 \\
%     Chinese             & ASR           & HKUST~\cite{liu06hkust}               & Telephone             & No        & 200 \\
%     Chinese             & ASR           & AISHELL-2~\cite{du18aishell2}         & In-house recording    & Yes       & 1,000 \\
%     Chinese             & ASV           & CN-Celeb~\cite{fan19cnceleb}          & bilibili.com          & Yes       & 1,000 \\
%     \end{tabular}
%     \label{tab:corpus_comparison}
% \end{table*}

==> tab/corpus_spec.tex <==
\begin{table}[t]
    \centering
    \caption{Results of data collection. Videos with automatic subtitles are not used in this paper, but the video ID is also opensourced.}
    \begin{tabular}{l|l}
        Retrieved entity                                & Value  \\ \hline
        \#search-terms                  & 2.34M terms \\
        \#videos found in the search    & 11.9M videos \\
        \#videos with manual subtitles  & 0.11M videos \\
        (\#videos with auto subtitles)  & 4.96M videos \\ 
    \end{tabular}
    \label{tab:corpus_spec}
    \vspace{-4mm}
\end{table}


% 多言語
% Librispeech
% Common Voice
% SPGISpeech
% Automatic Construction of a Large-Scale Speech Recognition Database Using Multi-Genre Broadcast Data with Inaccurate Subtitle Timestamps
% https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9414423
% https://arxiv.org/pdf/2104.04896.pdf
% https://arxiv.org/pdf/2006.08274.pdf と [10]


==> tab/video_type.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \caption{Comparison of classified and annotated video types.}
    \begin{tabular}{c|c|c|c}
    Classified \textbackslash Annotated   & TTS    & single speaker  & multi speakers \\ \hline
    TTS                     & 20     & 80       & 0 \\
    single speaker          & \textbf{5}      & \textbf{95}       & \textbf{0} \\
    multi speakers          & 1      & 36       & 63 \\
    \end{tabular}
    \vspace{-4mm}
    \label{tab:video_type}
\end{table}

==> temp_takamichi.tex <==
\newpage
\section{takamichi's memo (ato de kesu)}
    \textbf{Multi-speaker and noise-robust TTS.}
        Multi-speaker TTS uses speaker representations to control the speaker of the synthetic speech~\cite{DeepVoice2,DeepVoice3}. The $x$-vector used in automatic speaker verification (ASV) is an efficient approach for the control; we follow this in this paper. Also, a few-shot speaker adaptation, voice building of a new speaker from a small amount of speech data~\cite{cooperZeroShotMultiSpeakerEmbedding}, is the promising application of multi-speaker TTS. To increase the number of speakers using diverse training data, there exists some noise-aware TTS training~\cite{DenoiSpeech,DRSpeech,DenoiSpeech的なやつ}.
    
    \textbf{Building TTS corpus on ASR corpus.}
        The use of more speakers' data in training increases the speaker variation in TTS. Methods based on data refinement and selection of ASR corpora have been proposed for this purpose. The well-known examples are based on acoustic noise~\cite{話者認証からMultiSpeakerへの転移} and text label noise (i.e., a mismatch between text and speech)~\cite{LibriTTS}. These methodologies help construct a TTS corpus from an ASR corpus. However, these processes are based only on data quality and are performed independently of the TTS model. These methodologies are not appropriate considering the noise robustness of the TTS model, which we desribed above.
    
        Related to above, dark data has the potential to build massive speech corpora almost fully automatically, and indeed, successful examples of this have been reported in the construction of ASR corpora~\cite{galvez2021peoplespeech,chen2021gigaspeech}. In this paper, we focus on only the speaker variation but expect that it can be extended to other speech-related factors, e.g., style.
    
    \textbf{Prediction of perceptual quality in synthetic speech.}
        Methods for automatically predicting the subjective evaluation score from synthetic speech have been studied to reduce the evaluation cost for TTS~\cite{moller10mosprediction,patton16automos}. The challenge in automatic prediction is generalization performance, i.e., the robustness of the prediction against divergence between the training and evaluation data. The recent deep learning-based models (used in this paper) have relatively good accuracy in predicting the relative rank between speech samples, although the accuracy of predicting the value itself was reduced~\cite{huang22voicemos}.
        
